MISIM: A Neural Code Semantics Similarity System Using the Context-Aware Semantics Structure

Code semantics similarity can be used for many tasks such as code recommendation, automated software defect correction, and clone detection. Yet, the accuracy of such systems has not yet reached a level of general purpose reliability. To help address this, we present Machine Inferred Code Similarity (MISIM), a neural code semantics similarity system consisting of two core components: (i)MISIM uses a novel context-aware semantics structure, which was purpose-built to lift semantics from code syntax; (ii)MISIM uses an extensible neural code similarity scoring algorithm, which can be used for various neural network architectures with learned parameters. We compare MISIM to four state-of-the-art systems, including two additional hand-customized models, over 328K programs consisting of over 18 million lines of code. Our experiments show that MISIM has 8.08% better accuracy (using MAP@R) compared to the next best performing system.

==> Checklist.tex <==
\section*{Checklist}


\begin{enumerate}
    

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerNo{}
  \item Did you discuss any potential negative societal impacts of your work?
  \answerYes{They have been discussed in Appendix \ref{sect:impact}.}

  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}

\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Please see the supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{They are specified in the \textit{Training} paragraph in Section \ref{sect:experiments} and Appendix \ref{appendix:training}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Please see Figure \ref{fig:generalized_result} and Figure \ref{fig:spt_with_neural_backend}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We used POJ-104 and GCJ datasets, whose citations can be found in the \textit{Datasets} paragraph in Section \ref{sect:experiments}.}
  \item Did you mention the license of the assets?
    \answerNo{We have confirmed we are allowed to use the datasets. The POJ-104 dataset can be used freely for non-commercial purposes~\footnote{\url{https://sites.google.com/site/treebasedcnn}}, and the GCJ dataset is released under Apache License 2.0~\footnote{\url{https://github.com/Jur1cek/gcj-dataset}}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We included our code and filtered datasets in the supplemental material.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{
    We used publicly available data and were unable to check whether the consent was taken before collecting that data.
    }
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}
\end{enumerate}
